Reduction of turbulent skin-friction drag by passively rotating discs

A turbulent channel flow modified by the motion of discs that are free to rotate under the action of wall turbulence is studied numerically. The Navier-Stokes equations are coupled nonlinearly with the dynamical equation of the disc motion, which synthesizes the fluid-flow boundary conditions and is driven by the torque exerted by the wall-shear stress. We consider discs that are fully exposed to the fluid and discs for which only half of the surface interfaces the fluid. The disc motion is thwarted by the fluid torque in the housing cavity and by the torque of the ball bearing that supports the disc. For the full discs, no drag reduction occurs because of the small angular velocities. The most energetic disc response occurs for disc diameters that are comparable with the spanwise spacing of the low-speed streaks. A perturbation analysis for small disc-tip velocities reveals that the two-way nonlinear coupling has an intense attenuating effect on the disc response. The reduced-order results show excellent agreement with the nonlinear results for large diameters. The half discs rotate with a finite angular velocity, leading to large reduction of the turbulence activity and of the skin-friction drag over the spinning portion of the discs, while the maximum drag reduction over the entire walls is 5.6%. The dependence of the drag reduction on the wall-slip velocity and the spatial distribution of the wall-shear stress qualitatively match results based on the only available experimental data.

==> header.tex <==
\usepackage[T1]{fontenc}
\usepackage[scaled=0.85]{beramono}
\usepackage{geometry,graphicx,color,amsmath,amssymb}

% pgfplots/tikz :
\usepackage{tikz,tikzscale,pgfplots,etoolbox,pgfplotstable}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{colorbrewer}
\usepgfplotslibrary{colormaps}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}
\usetikzlibrary{arrows,calc,positioning,shapes,arrows,external,cd}
\tikzexternalize[prefix=./figs/build/]
\AtBeginEnvironment{tikzcd}{\tikzexternaldisable}
\AtEndEnvironment{tikzcd}{\tikzexternalenable}
%\pgfplotsset{compact=1.16}

% \usepackage{mathptmx}
\usepackage[font=small, justification=justified, width=\textwidth ,skip=2pt]{caption}
\usepackage{subcaption}
\usepackage{setspace}
\usepackage{float}
\usepackage{titlesec}
\usepackage{fancyhdr}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{natbib}
\usepackage{listings}
\usepackage{xfrac}
% \usepackage{hyperref}
\usepackage[colorlinks, citecolor=blue]{hyperref}
\usepackage{algorithmicx,algpseudocode,algorithm}
% \usepackage{lscape}
\usepackage{multirow}
\usepackage{lmodern}
\usepackage{verbatim}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathtools}
\usepackage{lmodern}
\usepackage{gensymb}
\usepackage{multirow}
\usepackage{url}
\usepackage{setspace}
\usepackage{natbib}
\usepackage[percent]{overpic}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{cancel}
\usepackage{soul}
\usepackage{float}
\usepackage{textcomp}
\usepackage{listings}
\usepackage{psfrag}
\usepackage{placeins}
\usepackage{color}
\usepackage{epsfig}
\usepackage{bm}
\usepackage{lscape}
\usepackage[usenames,dvipsnames,table]{xcolor}
\usepackage{tikz}
\usetikzlibrary{positioning,arrows}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{pstricks}
\usepackage[toc,page]{appendix}
\usepackage{upgreek}
\usepackage{caption}
\usepackage{multirow}
\usepackage[mathlines]{lineno}
\usepackage{scalerel}
\allowdisplaybreaks
\usepackage{anyfontsize}
\usepackage{mathrsfs}

%CLAUDIA'S THESIS
\usepackage{emptypage}
\usepackage{natbib}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{textcomp}
\usepackage{listings}
\usepackage{psfrag}
\usepackage{color}
\usepackage{epsfig,multirow}
\usepackage{bm,xparse}
\usepackage[intoc]{nomencl}
\usepackage[breaklinks=true]{hyperref}
\usepackage{lscape}
\usepackage[usenames,dvipsnames,table]{xcolor}
\usepackage{tikz,datetime}
%\usepackage{pdfpages}
\usepackage{verbatim}
\usepackage{float} 
\usepackage{subcaption}
\usepackage{epigraph}
\usepackage[shortlabels]{enumitem}
\usepackage{pgfplots}
\usetikzlibrary{spy}
\usetikzlibrary{decorations.markings}
\usepackage{cancel}
\usepackage{csquotes}
%\usepackage[titletoc]{appendix}
%\usepackage{paralist,enumitem}
\captionsetup[table]{justification=justified}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
% redefine titels format:
\titleformat*{\section}{\large\bfseries}
\titleformat*{\subsection}{\normalsize\bfseries}
\graphicspath{{./figs/}}

\pgfplotsset{
major tick length=0.08cm,
minor tick length=0.05cm,
every tick/.style={black,
semithick,
},
axis line style=semithick,
}
\pgfkeys{/pgf/number format/.cd,1000 sep={ }}

\usepackage[shortlabels]{enumitem}
\setlist[enumerate,1]{start=0}

% numbers subsubsections with letters:
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}
% \renewcommand{\thesubsubsection}{\thesubsection.\alph{subsubsection}}

% \pagestyle{fancy}
% \rhead{
% Notes free discs
% }
% \lhead{
% P. Olivucci
% }

\definecolor{schoolbusyellow}{rgb}{1.0, 0.85, 0.0}
\definecolor{folly}{rgb}{1.0, 0.0, 0.31}
\definecolor{electricindigo}{rgb}{0.44, 0.0, 1.0}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}

\numberwithin{equation}{section}
\numberwithin{figure}{section}

\usepackage[displaymath, mathlines]{lineno}
% \linenumbers

\makeatletter
\def\input@path{{./figs/}}
\makeatother
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> newcommands.tex <==
\newcommand{\gpathsmooth}{./figs/}
\newcommand{\gpathrings}{./figs/}
\newcommand{\gpathringsopp}{./figs/}
\newcommand{\gpathringslips}{./figs/}
\newtheorem{definition}{Definition}

\newcommand{\sca}{.4}
\newcommand{\gpath}{./figs/}

\newcommand{\plusref}{{0+}}


\newcommand{\mychar}[2]{%
  \begingroup\normalfont
  \raisebox{0.0em}{\includegraphics[height = #2]{#1}}
  \endgroup
}


\newcommand{\PLH}{{\mkern-2mu\times\mkern-2mu}}

\newcommand{\avertime}[1]{\overline{#1}}
\newcommand{\averensemble}[1]{\left[#1\right]_e}
\newcommand{\aversymmetry}[1]{\left[#1\right]_s}
\newcommand{\averspace}[1]{\langle #1 \rangle}
\newcommand{\averglobal}[1]{\left[#1\right]_g}

\newcommand{\xe}{x_e}
\newcommand{\ze}{z_e}
\newcommand{\xs}{x_s}
\newcommand{\zs}{z_s}

\newcommand{\blackline}{\raisebox{2pt}{\tikz{\draw[-,black!40!black,solid,line width = 0.7pt](0,0) -- (6mm,0);}}}
\newcommand{\solidline}[1]{\raisebox{2pt}{\tikz{\draw[-,#1,solid,line width = 0.7pt](0,0) -- (6mm,0);}}}
\newcommand{\dashline}[1]{\raisebox{2pt}{\tikz{\draw[-,#1,dashed,line width = 0.7pt](0,0) -- (6mm,0);}}}
\newcommand{\dotline}[1]{\raisebox{2pt}{\tikz{\draw[-,#1,dotted,line width = 0.7pt](0,0) -- (6mm,0);}}}
\newcommand{\dashdotline}[1]{\raisebox{2pt}{\tikz{\draw[-,#1,dashdotted,line width = 0.7pt](0,0) -- (6mm,0);}}}
\newcommand{\bluearrow}{\raisebox{2pt}{\tikz{\draw[->,blue,solid,line width = 0.7pt](0,0) -- (5mm,0);}}}
\newcommand{\circlec}[1]{\raisebox{0pt}{\tikz{\draw[#1,solid,line width = 0.7pt](0.mm,0) circle (0.75mm);}}}
\newcommand{\trianglec}[1]{\raisebox{0pt}{\tikz{\draw[#1,solid,line width = 0.7pt] (0,0) -- (0.2cm,0) -- (0.1cm,0.2cm) -- (0,0);}}}
\newcommand{\circles}[1]{\raisebox{0pt}{\tikz{\draw[#1,solid,fill=#1,line width = 0.7pt](0.mm,0) circle (0.75mm);}}}
\newcommand{\triangles}[1]{\raisebox{0pt}{\tikz{\draw[#1,solid,fill=#1,line width = 0.7pt] (0,0) -- (0.2cm,0) -- (0.1cm,0.2cm) -- (0,0);}}}
\newcommand{\rectanglec}[1]{\raisebox{0pt}{\tikz{\draw[#1,solid,line width = 0.7pt](2.mm,0) rectangle (3.5mm,1.5mm);}}}
\newcommand{\crossc}[1]{\raisebox{-1pt}{\tikz{\draw (0.,0.) node[cross out,draw=#1,rotate=45,line width = 0.7pt,minimum size=1.5mm,inner sep=0pt,outer sep=0pt] {};}}}
\newcommand{\crossx}[1]{\raisebox{0pt}{\tikz{\draw (0.,0.) node[cross out,draw=#1,rotate=0,line width = 0.7pt,minimum size=1.5mm,inner sep=0pt,outer sep=0pt] {};}}}


\newcommand{\solidc}[1]{\raisebox{0pt}{\tikz{\draw[fill=#1,#1](2.mm,0) rectangle (3.5mm,1.5mm);}}}
\definecolor{gold}{rgb}{.75,.75,0.}
\definecolor{cy}{rgb}{0.,.75,.75}
\definecolor{mag}{rgb}{.75,0.,.75}

\newcommand{\psfragnum}{
\psfrag{1}{1}
\psfrag{2}{2}
\psfrag{3}{3}
\psfrag{4}{4}
\psfrag{5}{5}
\psfrag{6}{6}
\psfrag{7}{7}
\psfrag{8}{8}
\psfrag{9}{9}
\psfrag{0}{0}
\psfrag{-}{-}
\psfrag{.}{.}
}

\newcommand{\totd}{D_{t}}
\newcommand{\p}{\partial}
\newcommand{\pdi}{\partial_{i}}
\newcommand{\pder}[3]{\frac{\partial^{#3} #1 }{{\partial #2}^{#3}}}
\newcommand{\pdj}{\partial_{j}}
\newcommand{\pddj}{\partial^{2}_{jj}}
\newcommand{\umi}{U_{i}}
\newcommand{\umj}{U_{j}}
\newcommand{\umk}{U_{k}}
\newcommand{\ui}{u_{i}}
\newcommand{\fcmi}{F_{i}}
\newcommand{\fci}{f_{i}}
\newcommand{\uj}{u_{j}}
\newcommand{\uk}{u_{k}}
\newcommand{\re}{\frac{1}{Re_p}}
\newcommand{\ommi}{\Omega_{i}}
\newcommand{\ommj}{\Omega_{j}}
\newcommand{\omi}{\omega_{i}}
\newcommand{\omj}{\omega_{j}}
\newcommand{\tlui}{\widetilde{u}_{i}}
\newcommand{\tluj}{\widetilde{u}_{j}}
\newcommand{\tlu}{\widetilde{u}}
\newcommand{\tlv}{\widetilde{v}}
\newcommand{\tlw}{\widetilde{w}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\br}[1]{\left\langle #1 \right\rangle}

\newcommand{\tbc}{{\color{magenta}$\spadesuit$}}

\newcommand{\includetikz}[1]{
    \tikzsetnextfilename{#1}
    \input{#1.tikz}%
}

%
%credits to https://tex.stackexchange.com/questions/67895/is-there-an-easy-way-of-using-line-thickness-as-error-indicator-in-a-plot
%
\newcommand{\errorband}[5][]{ % x column, y column, error column, optional argument for setting style of the area plot
\pgfplotstableread[col sep=space]{#2}\datatable
    % Lower bound (invisible plot)
    \addplot [draw=none, stack plots=y, forget plot] table [
        x index={#3},
        y expr=\thisrowno{#4}-\thisrowno{#5}
    ] {\datatable};

    % Stack twice the error, draw as area plot
    \addplot [draw=none, fill=gray!40, stack plots=y, area legend, #1] table [
        x index={#3},
        y expr=2*\thisrowno{#5}
    ] {\datatable} \closedcycle;

    % Reset stack using invisible plot
    \addplot [forget plot, stack plots=y,draw=none] table [x index={#3}, y expr=-(\thisrowno{#4}+\thisrowno{#5})] {\datatable};
}
